Global Weak Solutions for the Half-Wave Maps Equation in $\mathbb{R}$

We establish the existence of weak global solutions of the half-wave maps equation with the target $S^2$ on $\mathbb{R}^{1+1}$ with large initial data in $\dot{H}^1 \cap \dot{H}^{\frac{1}{2}}(\mathbb{R})$. We first prove the global well-posedness of a regularized equation. Then we show that the weak limit of the regularized solutions is a weak solution of the half-wave maps equation as the regularization parameter $\varepsilon \rightarrow 0$.

==> preamble.tex <==
%\usepackage[utf8]{inputenc}
%\usepackage[protrusion=allmath]{microtype}
\usepackage{afterpage}
\usepackage{lipsum}

\makeatletter
\newcommand{\oneraggedpage}{\let\mytextbottom\@textbottom
  \let\mytexttop\@texttop
  \raggedbottom
  \afterpage{%
  \global\let\@textbottom\mytextbottom
  \global\let\@texttop\mytexttop}}
  \usepackage{setspace}
\usepackage{color,soul}
\usepackage{float}
\usepackage{graphicx}
\usepackage{subfiles}
\usepackage{blindtext}
\graphicspath{ {/home/micatske/Semesterpaper} }
\usepackage{cite}
\usepackage{enumitem}
\usepackage{slashed}
%\usepackage{enumerate}
%\usepackage[title]{appendix}
%\usepackage[numbers]{natbib}
%\usepackage[nottoc]{tocbibind}
\usepackage[colorlinks=false,citecolor=black]{hyperref}
% For parsing options in custom notations (used in notation.tex)
\usepackage{xparse}
\usepackage{amsmath,stackengine}
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage{thm-restate}
%\declaretheorem{theorem}
\usepackage{amssymb}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{dsfont}
\usepackage{pgf,tikz}
\usepackage{mathrsfs}
\usepackage{xcolor}
\usepackage{hyperref} 
\usepackage{cleveref}
\usepackage{yfonts}
\usepackage{appendix}
\usepackage{cancel}
\usepackage{cite}
\usepackage{nth}
\usepackage{marginnote}
%\usepackage{pgfplots}
\usepackage{verbatim}
%\usepackage{latexsym,txfonts}
\hypersetup{backref=true,       
pagebackref=true,               
hyperindex=true,                
colorlinks=true,                
breaklinks=true,                
urlcolor= black,                
linkcolor= black,                
bookmarks=true,                 
bookmarksopen=false,
filecolor=black,
citecolor=black,
linkbordercolor=black
}
\usetikzlibrary{arrows}
\numberwithin{equation}{section}
\usetikzlibrary{patterns}


% List Environments
\iffalse

\usepackage[nottoc]{tocbibind}
\setlist{nolistsep}
\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother
\fi
% Theorem Environments
\swapnumbers
\theoremstyle{plain}
%\newtheorem{Theorem}{Theorem}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{Lemma}[theorem]{Lemma}
\newtheorem{Proposition}[theorem]{Proposition}
\newtheorem{Corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{Definition}[theorem]{Definition}
\newtheorem{Example}[theorem]{Example}
\newtheorem{Remark}[theorem]{Remark}
\newtheorem{Remarks}[theorem]{Remarks}
\newtheorem{Property}[theorem]{Property}
\newtheorem{Claim}[theorem]{Claim}
\newtheorem*{ack}{Acknowledgements}
%reptheorem
%\newtheorem*{rep@theorem}{\rep@title}
%\newcommand{\newreptheorem}[2]{%
%\newenvironment{rep#1}[1]{%
% \def\rep@title{#2 \ref{##1}}%
% \begin{rep@theorem}}%
% {\end{rep@theorem}}}
%\newreptheorem{theorem}{Theorem}
